QEVA: A Reference-Free Evaluation Metric for Narrative Video Summarization with Multimodal Question Answering

Video-to-text summarization remains underexplored in terms of comprehensive evaluation methods. Traditional n-gram overlap-based metrics and recent large language model (LLM)-based approaches depend heavily on human-written reference summaries, limiting their practicality and sensitivity to nuanced semantic aspects. In this paper, we propose QEVA, a reference-free metric evaluating candidate summaries directly against source videos through multimodal question answering. QEVA assesses summaries along three clear dimensions: Coverage, Factuality, and Chronology. We also introduce MLVU(VS)-Eval, a new annotated benchmark derived from the MLVU dataset, comprising 800 summaries generated from 200 videos using state-of-the-art video-language multimodal models. This dataset establishes a transparent and consistent framework for evaluation. Experimental results demonstrate that QEVA shows higher correlation with human judgments compared to existing approaches, as measured by Kendall's $\tau_b$, $\tau_c$, and Spearman's $\rho$. We hope that our benchmark and metric will facilitate meaningful progress in video-to-text summarization research and provide valuable insights for the development of future evaluation methods.

==> attachments/figure4.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{attachments/Capture 20250519_1430@2x.png}
    \caption{Methodology figure of QEVA.}
    \label{fig:qeva_pipeline}
    \end{figure*}
